Cut your Losses with Squentropy

Nearly all practical neural models for classification are trained using cross-entropy loss. Yet this ubiquitous choice is supported by little theoretical or empirical evidence. Recent work (Hui & Belkin, 2020) suggests that training using the (rescaled) square loss is often superior in terms of the classification accuracy. In this paper we propose the "squentropy" loss, which is the sum of two terms: the cross-entropy loss and the average square loss over the incorrect classes. We provide an extensive set of experiments on multi-class classification problems showing that the squentropy loss outperforms both the pure cross entropy and rescaled square losses in terms of the classification accuracy. We also demonstrate that it provides significantly better model calibration than either of these alternative losses and, furthermore, has less variance with respect to the random initialization. Additionally, in contrast to the square loss, squentropy loss can typically be trained using exactly the same optimization parameters, including the learning rate, as the standard cross-entropy loss, making it a true "plug-and-play" replacement. Finally, unlike the rescaled square loss, multiclass squentropy contains no parameters that need to be adjusted.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mixed loss functions/121_table_results.tex <==
\begin{table}[!htbp]
\centering
\vspace{-3mm}
\caption{Test accuracy (Acc)/ECE for 121 tabular datasets}
%\begin{threeparttable}
\label{121t1}
\begin{tabular}{|c|cc|cc|cc|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Squentropy}      & \multicolumn{2}{c|}{Cross-entropy} & \multicolumn{2}{c|}{Rescaled square} \\ \cline{2-7} 
                         & \multicolumn{1}{c}{Acc}       & ECE & \multicolumn{1}{c}{Acc}   & ECE   & \multicolumn{1}{c}{Acc}  & ECE  \\ \hline
abalone & 66.0 & \textbf{3.9} & 67.9 & 14.1 & \textbf{68.3} & 13.8 \\ \hline 
acute-inflammation & \textbf{96.4} & \textbf{3.8} & 91.3 & 4.7 & 95.8 & 4.3 \\ \hline 
acute-nephritis & \textbf{100.0} & \textbf{1.7} & \textbf{100.0} & 3.0 & \textbf{100.0} & 4.8 \\ \hline 
adult & 84.0 & \textbf{4.7} & \textbf{85.1} & 5.7 & \textbf{85.1} & 10.7 \\ \hline 
annealing & 94.3 & \textbf{3.6} & 93.3 & 3.9 & \textbf{94.4} & 4.1 \\ \hline 
arrhythmia & 68.1 & 21.4 & 67.0 & 24.5 & \textbf{68.4} & \textbf{17.3} \\ \hline 
audiology-std & 72.6 & 26.3 & \textbf{73.0} & \textbf{26.0} & 70.3 & 29.7 \\ \hline 
balance-scale & \textbf{97.2} & 5.0 & 96.3 & \textbf{3.8} & 96.5 & 4.0 \\ \hline 
balloons & \textbf{95.6} & 23.7 & 95.4 & \textbf{21.4} & 90.0 & 25.8 \\ \hline 
bank & \textbf{89.9} & \textbf{4.1} & 89.8 & 7.7 & 89.2 & 10.6 \\ \hline 
blood & 81.6 & 11.7 & \textbf{81.9} & \textbf{7.0} & 81.7 & 16.6 \\ \hline 
breast-cancer & \textbf{76.8} & 26.6 & 75.6 & \textbf{24.5} & 75.5 & 27.5 \\ \hline 
breast-cancer-wisc & \textbf{98.0} & 4.8 & 97.6 & 4.9 & 97.1 & \textbf{4.5} \\ \hline 
breast-cancer-wisc-diag & \textbf{99.5} & 3.5 & 99.2 & 3.4 & 98.8 &\textbf{ 2.2} \\ \hline 
breast-cancer-wisc-prog & \textbf{89.6} & 16.3 & 87.9 & \textbf{15.7} & 89.0 & 19.3 \\ \hline 
breast-tissue & 83.3 & 17.9 & \textbf{84.1} & \textbf{17.1} & 83.6 & 19.2 \\ \hline 
car & \textbf{100.0} & \textbf{0.4} & \textbf{100.0} & \textbf{0.4} & \textbf{100.0} & 2.3 \\ \hline 
cardiotocography-10clases & 87.7 & 6.3 & \textbf{87.8} & 7.3 & 87.2 & \textbf{3.9} \\ \hline 
cardiotocography-3clases & 94.8 & \textbf{4.0} & \textbf{94.9} & 5.5 & 94.7 & 4.6 \\ \hline 
chess-krvk & 86.6 & 3.7 & \textbf{87.8} & \textbf{1.8} & 86.1 & 16.0 \\ \hline 
chess-krvkp & \textbf{99.8} & \textbf{0.4} & 99.7 & 0.5 & \textbf{99.8} & 0.7 \\ \hline 
congressional-voting & \textbf{65.9} & 9.7 & 65.7 & \textbf{9.2} & 65.1 & 18.3 \\ \hline 
conn-bench-sonar-mines-rocks & 90.6 & 11.7 & \textbf{91.4} & \textbf{10.2} & \textbf{91.4} & 13.1 \\ \hline 
conn-bench-vowel-deterding & \textbf{99.6} & 2.7 & 99.1 & \textbf{1.9} & 98.9 & 9.3 \\ \hline 
connect-4 & 89.4 & \textbf{3.3} & 89.0 & 5.1 & \textbf{89.7} & 6.6 \\ \hline 
contrac & 57.7 & \textbf{13.6} & 58.6 & 30.4 & \textbf{58.0} & 35.3 \\ \hline 
credit-approval & \textbf{89.1} & \textbf{9.4} & 88.4 & 11.7 & 88.6 & 14.3 \\ \hline 
cylinder-bands & 81.9 & \textbf{13.1} &\textbf{ 84.1} & 14.8 & 83.9 & 17.8 \\ \hline 
dermatology & \textbf{97.6} & 4.7 & 97.2 & 4.4 & 97.3 & \textbf{3.5} \\ \hline 
echocardiogram & \textbf{85.0} & \textbf{17.6} & 84.9 & 17.8 & 84.4 & 19.3 \\ \hline 
ecoli & \textbf{88.2} & 12.4 & 88.1 & \textbf{7.8} & \textbf{88.2} & 9.8 \\ \hline 
energy-y1 & 97.3 & 4.2 & \textbf{97.5} & 4.2 & 97.3 & \textbf{3.0} \\ \hline 
energy-y2 & \textbf{97.2} & 4.4 & 96.7 & 5.3 & 96.4 & \textbf{4.0} \\ \hline 
fertility & \textbf{94.6} & 23.3 & 93.4 & 26.3 & 90.0 & \textbf{19.4} \\ \hline 
flags & \textbf{60.1} & 27.1 & 58.4 & 31.3 & 57.4 & \textbf{20.6} \\ \hline 
glass & \textbf{78.7} & \textbf{18.7} & 78.1 & 25.4 & 78.1 & 20.8 \\ \hline 
haberman-survival & \textbf{80.3} & \textbf{12.2} & 79.8 & 17.9 & 79.7 & 22.9 \\ \hline 
hayes-roth & \textbf{85.8} & \textbf{5.4} & 84.1 & 11.4 & 83.7 & 13.6 \\ \hline 
heart-cleveland & 62.5 & 32.0 & 62.1 & 32.5 & \textbf{64.6} & \textbf{25.7} \\ \hline 
heart-hungarian & 85.3 & 17.6 & 84.8 & \textbf{16.0} & \textbf{85.4} & 19.2 \\ \hline 
heart-switzerland & 43.8 & 50.4 & 43.6 & 47.7 & \textbf{46.4} &\textbf{ 44.4} \\ \hline 
heart-va & 42.1 & \textbf{46.0} & \textbf{46.4} & 54.1 & 42.0 & 47.9 \\ \hline 
hepatitis & 77.4 & 18.1 & 75.3 & 20.6 & \textbf{84.5} & \textbf{14.8} \\ \hline 
hill-valley & 66.0 & \textbf{14.2} & \textbf{71.9} & 36.3 & 71.1 & 40.2 \\ \hline 
horse-colic & 85.9 & \textbf{13.3} & 84.4 & 13.9 & \textbf{86.0} & 14.2 \\ \hline 

\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\vspace{-3mm}
\caption{Test accuracy (Acc)/ECE for 121 tabular datasets}
%\begin{threeparttable}
\label{121t2}
\begin{tabular}{|c|cc|cc|cc|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Squentropy}      & \multicolumn{2}{c|}{Cross-entropy} & \multicolumn{2}{c|}{Rescaled square} \\ \cline{2-7} 
                         & \multicolumn{1}{c}{Acc}       & ECE & \multicolumn{1}{c}{Acc}   & ECE   & \multicolumn{1}{c}{Acc}  & ECE  \\ \hline
ilpd-indian-liver & \textbf{77.2} & \textbf{12.7} & 75.3 & 22.9 & 75.9 & 25.7 \\ \hline 
image-segmentation & \textbf{96.8} & \textbf{5.4} & 94.7 & 6.5 & 94.8 & 6.9 \\ \hline 
ionosphere & \textbf{98.3} & 7.0 & 98.2 &\textbf{ 5.5} & 97.2 & 6.2 \\ \hline 
iris & 97.2 & 3.9 & 97.1 & 4.3 & \textbf{98.0} & \textbf{2.9} \\ \hline 
led-display & 75.2 & 10.7 & \textbf{75.3} & \textbf{5.2} & 74.9 & 8.3 \\ \hline 
lenses & 76.6 & 20.8 & 68.4 & 21.5 & \textbf{80.0} & \textbf{17.8} \\ \hline 
letter & \textbf{98.8} & \textbf{1.1} & 98.6 & 1.2 & 98.4 & 16.6 \\ \hline 
libras & \textbf{93.1} & \textbf{4.9} & 92.9 & 5.7 & 92.5 & 12.9 \\ \hline 
low-res-spect & \textbf{95.9} & \textbf{4.0} & 95.2 & 5.0 & 94.2 & 7.7 \\ \hline 
lung-cancer & 60.6 & \textbf{27.1} & 54.7 & 40.4 & \textbf{62.9} & 40.4 \\ \hline 
lymphography & 89.2 & \textbf{6.4} & 87.1 & 7.1 & \textbf{91.3} & 8.0 \\ \hline 
magic & 88.3 & 5.5 & 89.1 & \textbf{5.3} & \textbf{89.2} & 8.3 \\ \hline 
mammographic & 81.9 & 9.4 & 83.3 & \textbf{8.0} & \textbf{83.4} & 14.6 \\ \hline 
miniboone & \textbf{81.7} & \textbf{20.3} & 81.5 & \textbf{20.3} & 77.9 & 27.2 \\ \hline 
molec-biol-promoter & \textbf{87.9} & 11.4 & 78.6 & \textbf{9.9} & 85.5 & 14.8 \\ \hline 
molec-biol-splice & \textbf{87.9} & \textbf{7.1} & 84.2 & 10.8 & 87.2 & 8.2 \\ \hline 
monks-1 & 85.4 & 14.0 & 83.6 & \textbf{13.5} & \textbf{87.2} & 14.6 \\ \hline 
monks-2 & 72.9 & \textbf{6.9} & 89.9 & 12.8 & \textbf{95.9} & 14.5 \\ \hline 
monks-3 & \textbf{93.4} & \textbf{6.7} & 91.6 & 7.6 & 92.0 & 9.4 \\ \hline 
mushroom & \textbf{100.0} & \textbf{0.0} & \textbf{100.0} & \textbf{0.0} & \textbf{100.0} & 0.7 \\ \hline 
musk-1 & 95.2 & \textbf{3.3} & 94.6 & 6.3 & \textbf{95.6} & 4.9 \\ \hline 
musk-2 & \textbf{100.0} & 1.1 & \textbf{100.0} & 0.2 & \textbf{100.0} & \textbf{0.7} \\ \hline 
nursery & \textbf{100.0} & 0.1 & \textbf{100.0} & \textbf{0.0} & \textbf{100.0} & 2.7 \\ \hline 
oocytes\_merluccius\_nucleus\_4d & 85.1 & \textbf{3.5} & 86.6 & 10.4 & \textbf{87.1} & 14.4 \\ \hline 
oocytes\_merluccius\_states\_2f & \textbf{95.4} & \textbf{3.2} & 95.2 & 6.3 & 95.2 & 4.6 \\ \hline 
oocytes\_trisopterus\_nucleus\_2f & 89.0 & \textbf{5.4} & \textbf{89.7} & 9.2 & 89.0 & 10.7 \\ \hline 
oocytes\_trisopterus\_states\_5b & 97.1 & 4.3 & 97.1 & 4.6 & \textbf{97.3} & \textbf{3.7} \\ \hline 
optical & \textbf{99.6} & \textbf{0.9} & 99.3 & 1.2 & 99.0 & 6.6 \\ \hline 
ozone & \textbf{97.7} & 4.5 & 97.5 & 3.9 & 97.1 & \textbf{3.1} \\ \hline 
page-blocks & \textbf{97.7} & 2.2 & 97.5 & 2.3 & 97.1 & \textbf{1.8} \\ \hline 
parkinsons & 97.0 & \textbf{2.9} & \textbf{97.9} & 5.8 & 97.4 & 4.2 \\ \hline 
pendigits & 99.8 & \textbf{0.2} & 99.8 & 0.3 & \textbf{99.9} & 6.1 \\ \hline 
pima & \textbf{79.9} & \textbf{20.8} & 78.0 & 22.4 & 77.4 & 24.6 \\ \hline 
pittsburg-bridges-MATERIAL & 79.7 & 15.4 & 80.4 & 15.8 & \textbf{89.1} & \textbf{14.0} \\ \hline 
pittsburg-bridges-REL-L & 68.2 & 30.2 & 66.2 & \textbf{28.3} & \textbf{73.3} & 36.5 \\ \hline 
pittsburg-bridges-SPAN & 73.2 & 31.0 & 69.9 & \textbf{30.8} & \textbf{73.7} & 34.6 \\ \hline 
pittsburg-bridges-T-OR-D & \textbf{90.1} & 19.3 & 90.0 & 24.5 & 89.5 & \textbf{17.9} \\ \hline 
pittsburg-bridges-TYPE & 63.4 & 34.8 & 63.3 & \textbf{33.0} & \textbf{66.7} & 39.7 \\ \hline 
planning & \textbf{77.9} & \textbf{23.4} & 75.6 & 33.5 & 76.8 & 31.7 \\ \hline 
plant-margin & \textbf{85.1} & \textbf{4.4} & 84.0 & 5.9 & 82.9 & 55.7 \\ \hline 
plant-shape & \textbf{74.3} & \textbf{7.8} & 73.9 & 13.9 & 70.6 & 49.1 \\ \hline 
plant-texture & \textbf{85.3} & \textbf{3.1} & 84.3 & 6.2 & 82.6 & 52.8 \\ \hline 
post-operative & \textbf{73.9} & 35.2 & 70.4 & \textbf{34.7} & 62.2 & 35.3 \\ \hline 
primary-tumor & \textbf{50.0} & 27.7 & 49.8 & 38.5 & 48.5 & \textbf{24.0} \\ \hline 
ringnorm & \textbf{98.6} & 1.7 & 98.5 & 2.1 & 98.1 & \textbf{1.5} \\ \hline 

\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\vspace{-3mm}
\caption{Test accuracy (Acc)/ECE for 121 tabular datasets}
\label{121t3}

\begin{tabular}{|c|cc|cc|cc|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Squentropy}      & \multicolumn{2}{c|}{Cross-entropy} & \multicolumn{2}{c|}{Rescaled square} \\ \cline{2-7} 
                         & \multicolumn{1}{c}{Acc}       & ECE & \multicolumn{1}{c}{Acc}   & ECE   & \multicolumn{1}{c}{Acc}  & ECE  \\ \hline
seeds & \textbf{100.0} & \textbf{4.0} & 99.0 & 6.3 & 98.6 & 5.9 \\ \hline 
semeion & \textbf{95.4} & \textbf{2.3} & 94.9 & 3.5 & 94.8 & 10.7 \\ \hline 
soybean & \textbf{92.2} & \textbf{3.4} & 90.8 & 3.9 & 91.3 & 17.5 \\ \hline 
spambase & \textbf{95.6} & \textbf{4.1} & 95.4 & 4.6 & 95.0 & 4.9 \\ \hline 
spect & \textbf{76.8} & \textbf{37.3} & 75.4 & 41.7 & 76.2 & 42.2 \\ \hline 
spectf & 79.3 & 18.2 & 82.9 & \textbf{17.1} & \textbf{83.8} & 21.8 \\ \hline 
statlog-australian-credit & 61.2 & \textbf{24.1} & 64.5 & 34.0 & \textbf{66.4} & 34.1 \\ \hline 
statlog-german-credit & \textbf{80.3} & \textbf{15.7} & 79.1 & 21.2 & 79.6 & 23.1 \\ \hline 
statlog-heart & \textbf{86.9} & 18.0 & 86.4 & \textbf{15.4} & 85.9 & 18.8 \\ \hline 
statlog-image & \textbf{99.3} & \textbf{1.4} & 99.1 & \textbf{1.4} & 98.8 & 4.1 \\ \hline 
statlog-landsat & \textbf{93.3} & 5.8 & 93.0 & 6.8 & 92.7 & \textbf{2.7} \\ \hline 
statlog-shuttle & \textbf{99.8} & \textbf{0.5} & \textbf{99.8} & \textbf{0.5} & \textbf{99.8} & 3.7 \\ \hline 
statlog-vehicle & \textbf{87.5} & \textbf{7.8} & 86.9 & 9.7 & 86.8 & 11.9 \\ \hline 
steel-plates & \textbf{78.8} & \textbf{9.7} & 78.5 & 14.4 & 78.7 & 10.2 \\ \hline 
synthetic-control &\textbf{ 99.1} & 2.1 & \textbf{99.1} & \textbf{2.0} & 98.7 & 4.9 \\ \hline 
teaching & \textbf{65.1} & \textbf{29.9} & 63.0 & 30.5 & 63.9 & 37.2 \\ \hline 
thyroid & \textbf{98.5} & 2.0 & 97.6 & 2.6 & 97.9 & \textbf{1.4} \\ \hline 
tic-tac-toe & \textbf{99.8} & 0.3 & \textbf{99.8} & \textbf{0.2} & \textbf{99.8} & 0.6 \\ \hline 
titanic & 78.6 & 12.6 & 78.4 & \textbf{4.2} & \textbf{78.9} & 13.6 \\ \hline 
trains &\textbf{ 100.0} & 34.1 & 90.4 & \textbf{27.2} & 80.0 & 53.0 \\ \hline 
twonorm & \textbf{98.2} & \textbf{2.0} & 98.1 & 2.6 & 97.7 & \textbf{2.0} \\ \hline 
vertebral-column-2clases & 91.2 & \textbf{8.5} & 91.1 & 8.6 & \textbf{91.3} & 13.1 \\ \hline 
vertebral-column-3clases & \textbf{88.0} & 15.4 & 86.6 & \textbf{15.1} & 87.1 & 16.1 \\ \hline 
wall-following & \textbf{96.1} & 2.2 & 95.8 & 3.2 & 95.7 & \textbf{1.7} \\ \hline 
waveform & 86.5 & \textbf{9.0} & 86.8 & 11.2 & \textbf{86.9} & 12.0 \\ \hline 
waveform-noise & 85.4 & \textbf{9.4} & 85.4 & 11.9 & \textbf{86.1} & 14.1 \\ \hline 
wine & \textbf{100.0} & 3.3 & \textbf{100.0} & 3.0 & \textbf{100.0} & \textbf{2.9} \\ \hline 
wine-quality-red & 68.8 & 23.2 & 68.9 & 26.6 & \textbf{69.3} & \textbf{19.7} \\ \hline 
wine-quality-white & 65.0 & 19.9 & \textbf{65.9} & 25.3 & 65.5 & \textbf{17.2} \\ \hline 
yeast & 63.3 & 21.4 & 63.1 & 29.9 & \textbf{63.5} & \textbf{18.8} \\ \hline 
zoo & \textbf{92.0} & 4.8 & 91.9 & \textbf{3.9} & 91.4 & 9.1 \\ \hline 

\end{tabular}
\end{table}


==> mixed loss functions/accuracy_ece.tex <==
\begin{table*}[ht]
\centering
\vspace{-3mm}
\caption{Test performance (\textbf{perf}(\%): accuracy for NLP\&Vision, error rate for speech data) and calibration: \textbf{ECE}(\%).}
\label{acc_ece}
%\begin{threeparttable}

\begin{tabular}{ccccccccc}
\hline
\hline
\multirow{2}{*}{Domain}   & \multirow{2}{*}{Model}                               & \multirow{2}{*}{Task}            & \multicolumn{2}{c}{Squentropy} & \multicolumn{2}{c}{Cross-entropy} &\multicolumn{2}{c}{Square loss}  \\ \cline{4-9}
&         &              & \multicolumn{1}{c|}{perf} & ECE & \multicolumn{1}{c|}{perf} &ECE &  \multicolumn{1}{c|}{perf} &ECE \\ \hline
\multirow{15}{*}{NLP} & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}fine-tuned BERT \\\cite{devlin2018bert}\end{tabular}} & MRPC &  \multicolumn{1}{c|}{$\textbf{84.0}$}&$\textbf{7.9}$ &    \multicolumn{1}{c|}{$82.1$}& $13.1$   & \multicolumn{1}{c|}{$83.8$}&$14.0$\\
                              &    & SST-2   &   \multicolumn{1}{c|}{$\textbf{94.2}$}&$7.0$               & \multicolumn{1}{c|}{$93.9$}&$\textbf{6.7}$  & \multicolumn{1}{c|}{$94.0$}&$19.8$ \\
                             &     & QNLI     &  \multicolumn{1}{c|}{$\textbf{91.0}$}&$7.3$         & \multicolumn{1}{c|}{$90.6$}&$7.4$  & \multicolumn{1}{c|}{$90.6$ }&$\textbf{4.2}$\\
                           &       & QQP &    \multicolumn{1}{c|}{$\textbf{89.0}$} & $\textbf{2.2}$        & \multicolumn{1}{c|}{$88.9$}&$5.8$   &\multicolumn{1}{c|}{$88.9$} & $2.8$ \\
                           &       & text5 & \multicolumn{1}{c|}{$\textbf{85.2}$}&$\textbf{12.4}$ &\multicolumn{1}{c|}{$84.5$}&$14.9$     & \multicolumn{1}{c|}{$84.6$}&$46.7$\\
                           &       & text20   &  \multicolumn{1}{c|}{$\textbf{81.2}$}&$\textbf{10.5}$                 & \multicolumn{1}{c|}{$80.8$}&$16.2$ & \multicolumn{1}{c|}{$80.8$}&$69.2$ \\
                                  \cline{2-9}

& \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL \\ \cite{dai2019transformer}\end{tabular}} & text8 &  \multicolumn{1}{c|}{$71.5$}&$\textbf{3.9}$  &    \multicolumn{1}{c|}{$\textbf{72.8}$}&$5.8$   & \multicolumn{1}{c|}{$73.2$}&$57.6$\\
                          &        & enwik8   &    \multicolumn{1}{c|}{$77.0$}& $\textbf{4.8}$           & \multicolumn{1}{c|}{$\textbf{77.5}$}&$9.3$  & \multicolumn{1}{c|}{$76.7$}&$64.5$ \\
                         &         & enwik8 (subset) & \multicolumn{1}{c|}{$\textbf{48.9}$}&$\textbf{10.7}$  & \multicolumn{1}{c|}{$48.6$}&$18.9$ & \multicolumn{1}{c|}{$47.3$}&$70.6$  \\
                                   \cline{2-9}
&\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention  \\ \cite{chen2016enhanced} \end{tabular}}              & MRPC&   \multicolumn{1}{c|}{$71.4$}&$\textbf{3.2}$ & \multicolumn{1}{c|}{$70.9$}&$7.1$   & \multicolumn{1}{c|}{$\textbf{71.7}$}&$3.5$\\
                          &        & QNLI &  \multicolumn{1}{c|}{$\textbf{79.3}$}&$\textbf{7.2}$    & \multicolumn{1}{c|}{$79.0$}&$7.6$     &\multicolumn{1}{c|}{$\textbf{79.3}$}&$13.0$ \\
                            &      & QQP  &  \multicolumn{1}{c|}{$\textbf{83.5}$}&$\textbf{2.4}$    & \multicolumn{1}{c|}{$83.1$}&$3.2$        &    \multicolumn{1}{c|}{ $\textbf{83.4}$}&$16.5$ \\ \cline{2-9}
&\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \cite{he2016pairwise}\end{tabular}}          & MRPC&    \multicolumn{1}{c|}{$70.5$}&$\textbf{5.2}$               &      \multicolumn{1}{c|}{ $69.4$} & $6.3$  &   \multicolumn{1}{c|}{$\textbf{73.2}$}&$16.3$   \\
                          &        & QNLI &  \multicolumn{1}{c|}{$\textbf{76.0}$}&$4.1$                   &    \multicolumn{1}{c|}{$\textbf{76.0}$}&$\textbf{2.3}$ & \multicolumn{1}{c|}{$\textbf{76.0}$}&$20.5$ \\&
                                  & QQP  &   \multicolumn{1}{c|}{$\textbf{84.5}$}&$\textbf{5.1}$                &   \multicolumn{1}{c|}{$84.4$}&$7.2$ &\multicolumn{1}{c|}{ $84.3$}&$24.6$ \\ \hline

\multirow{8}{*}{Speech} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Attention+CTC \\ \cite{kim2017joint} \end{tabular}} & TIMIT (PER)  &  \multicolumn{1}{c|}{$\textbf{19.6}$}&$\textbf{0.7}$ & \multicolumn{1}{c|}{$20.0$}&$3.1$  &    \multicolumn{1}{c|}{$20.0$}&$2.8$       \\
& & TIMIT (CER)  & \multicolumn{1}{c|}{$\textbf{32.1}$}&$\textbf{1.6}$   & \multicolumn{1}{c|}{$33.4$}&$3.3$ &    \multicolumn{1}{c|}{$32.5$}&$4.3$       \\
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTMP  \\ \cite{moritz2019triggered}
 \end{tabular}}  & WSJ (WER) & \multicolumn{1}{c|}{$5.5$}&$\textbf{3.2}$   &  \multicolumn{1}{c|}{$5.3$}&$5.0$ & \multicolumn{1}{c|}{$\textbf{5.1}$}&$5.3$ \\
 & & WSJ (CER) &  \multicolumn{1}{c|}{$2.9$}&$\textbf{3.2}$   & \multicolumn{1}{c|}{$2.5$}&$5.0$ & \multicolumn{1}{c|}{$\textbf{2.4}$}&$5.3$ \\
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTM \\ 
\cite{moritz2019triggered} \end{tabular}}& Librispeech (WER)   & \multicolumn{1}{c|}{$\textbf{7.6}$}&$7.1$    & \multicolumn{1}{c|}{$8.2$}&$\textbf{2.7}$ & \multicolumn{1}{c|}{ $8.0$}&$7.9$  \\ 
& & Librispeech (CER)  & \multicolumn{1}{c|}{$\textbf{9.7}$}&$ 7.1 $    &  \multicolumn{1}{c|}{$10.6$}&$ \textbf{2.7} $  &  \multicolumn{1}{c|}{$\textbf{9.7}$}&$ 7.9 $ \\
% & & Librispeech (SER)  & \multicolumn{1}{c|}{$\textbf{69.2}$}&$-$    & \multicolumn{1}{c|}{ $71.5$}&$-$  &  \multicolumn{1}{c|}{$69.4$}&$-$ \\
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Transformer \\ \cite{watanabe2018espnet} \end{tabular}}    & WSJ (WER)         &  \multicolumn{1}{c|}{$\textbf{3.9}$}&$\textbf{2.1}$ &  \multicolumn{1}{c|}{$4.2$}&$4.3$  &  \multicolumn{1}{c|}{$4.0$}&$4.4$     \\
& & Librispeech (WER)  &\multicolumn{1}{c|}{$\textbf{9.1}$}&$\textbf{4.2}$     & \multicolumn{1}{c|}{$9.2$}&$4.9$ & \multicolumn{1}{c|}{$9.4$}&$5.1$  \\  \hline
\multirow{11}{*}{Vision} & TCNN \cite{bai2018empirical}   & MNIST      &    \multicolumn{1}{c|}{$\textbf{97.8}$}&$\textbf{1.4}$   & \multicolumn{1}{c|}{$97.7$}&$1.6$    &       \multicolumn{1}{c|}{$97.7$}&$75.0$   \\ 
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Resnet-18 \\ \cite{he2016deep} \end{tabular}} & CIFAR-10  & \multicolumn{1}{c|}{$\textbf{85.5}$}&$\textbf{8.9}$  & \multicolumn{1}{c|}{$84.7$}&$10.0$  & \multicolumn{1}{c|}{$84.6$}&$13.4$ \\ 
& & STL-10 &  \multicolumn{1}{c|}{$93.0$}&$\textbf{21.2}$ & \multicolumn{1}{c|}{$\textbf{93.7}$}&$26.1$  & \multicolumn{1}{c|}{$92.5$}&$40.3$ \\
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} W-Resnet \\ \cite{zagoruyko2016wide}\end{tabular}} & CIFAR-100 & \multicolumn{1}{c|}{$\textbf{77.5}$} & $\textbf{10.9}$ & \multicolumn{1}{c|}{$76.7$}  &$17.9$ & \multicolumn{1}{c|}{$76.5$ }&$12.7$\\
& & CIFAR-100 (subset) & \multicolumn{1}{c|}{$\textbf{43.5}$}&$\textbf{18.8}$ & \multicolumn{1}{c|}{$41.5$}&$40.3$ & \multicolumn{1}{c|}{$41.0$}&$23.8$ \\
&Visual transformer  & CIFAR-10  & \multicolumn{1}{c|}{$\textbf{99.3}$}&$\textbf{1.9}$   & \multicolumn{1}{c|}{$99.2$}&$3.8$  &   \multicolumn{1}{c|}{$\textbf{99.3}$}&$7.2$\\ 
&VGG & SVHN  & \multicolumn{1}{c|}{$67.7$}&$\textbf{4.8}$ & \multicolumn{1}{c|}{$\textbf{68.9}$}&$5.7$  & \multicolumn{1}{c|}{$67.0$}&$65.4$ \\

\cline{2-9}
&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Resnet-50 \\ \cite{he2016deep}\end{tabular}}    & ImageNet (acc.)       & \multicolumn{1}{c|}{ $\textbf{76.3}$}& $\textbf{6.3}$  & \multicolumn{1}{c|}{$76.1$}&$6.7$  &     \multicolumn{1}{c|}{ $ 76.2$}& 8.2 \\
& & ImageNet (Top-5 acc.) &\multicolumn{1}{c|}{$ \textbf{93.2}$} &N/A & \multicolumn{1}{c|}{$93.0$}&N/A &     \multicolumn{1}{c|}{ $93.0$}&N/A \\
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}EfficientNet \\ \cite{tan2019efficientnet}\end{tabular}} & ImageNet (acc.)       &  \multicolumn{1}{c|}{$76.4$}&  $6.8$  & \multicolumn{1}{c|}{$\textbf{77.0}$}&   $\textbf{5.6}$  & \multicolumn{1}{c|}{$74.6$}&   $7.9$   \\
& & ImageNet (Top-5 acc.) & \multicolumn{1}{c|}{$93.0$}&N/A   & \multicolumn{1}{c|}{$\textbf{93.3}$}&N/A&     \multicolumn{1}{c|}{$92.7$}&N/A\\ \hline
\end{tabular}
% \begin{tablenotes}[para,flushleft]
% \label{TER}
% \item [$*$] For WSJ, WER shares the same acoustic model with CER, the calibration numbers are the same for CER. Similarly, WER, CER and SER of Librispeech shares the same acoustic model, hence only one calibration results. 
% \item[$^\diamondsuit$]For Top-5 accuracy,  the ECE numbers are not available.
% \end{tablenotes}
% \end{threeparttable}
\vspace{-2mm}
\end{table*}

==> mixed loss functions/ece_plots.tex <==
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/text5_diag.pdf}} 
\vspace{-15mm}
\caption{Reliability diagrams for a pretrained BERT
on text5 data. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/text20_diag.pdf}} 
\vspace{-15mm}
\caption{Reliability diagrams for a pretrained BERT
on text20 data. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/enwik8_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a Transformer-XL
on enwik8. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/text8_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a Transformer-XL
on text8. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/TIMIT_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a Attention+CTC model
on TIMIT. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}

\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/WSJ_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a VGG+BLSTMP model
on WSJ. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} scaled square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/Librispeech_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a VGG+BLSTM model
on Librispeech. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} scaled square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/MNIST_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a TCN
on MNIST. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}


\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/CIFAR-10_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a Resnet18
on CIFAR-10.\textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} scaled square loss.}
\end{figure*}


\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/CIFAR-100_subset_diag.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a Wide Resnet
on CIFAR-100 subset. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} scaled square loss.}
\end{figure*}

\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/STL-10_diag1.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a Resnet18
on STL10. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}
\begin{figure*}[!htbp]
  % \centering
\centerline{\includegraphics[width=1\columnwidth]{figs/SVHN_diag1.pdf}} 
\vspace{-15mm}
  \caption{Reliability diagrams for a VGG
on SVHN. \textit{Left:} squentropy, \textit{middle:} cross-entropy, \textit{right:} square loss.}
\end{figure*}

==> mixed loss functions/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mixed loss functions/para.tex <==
\begin{table}[!ht]
\centering
\vspace{-2mm}
\caption{Hyper-parameters for CIFAR-100, SVHN, and STL-10.}
\label{vision_para}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Task} & \multirow{2}{*}{Hyper-parameters} & \multicolumn{3}{c|}{Epochs training w/} \\ \cline{4-6} 
                       &                       &                           &squentropy        & square loss           & CE              \\ \hline

Wide-ResNet            & CIFAR-100              &   \begin{tabular}[c]{@{}c@{}}   lr=0.1, layer=28 \\ wide-factor=20, batch size: 128    \end{tabular}                         & 200            &200       & 200             \\ \hline
VGG             & SVHN              &   \begin{tabular}[c]{@{}c@{}} lr=0.1 for cross-entropy\\lr=0.0.02 for squentropy and square loss\end{tabular}                                & 200                & 200 &200         \\ \hline
Resnet-18           & STL-10              & \begin{tabular}[c]{@{}c@{}} lr=0.1 for cross-entropy\\ for squentropy and square loss lr=0.02                 \end{tabular}               & 200 &200              & 200           \\ \hline
\end{tabular}
\end{threeparttable}
\vspace{-4mm}
\end{table}

==> mixed loss functions/variance.tex <==
\begin{table}[!htbp]
\centering
\vspace{-4mm}
\caption{Standard deviation of test accuracy/error. Smaller number is bolded. CE is short for cross-entropy.} 
\label{variance}
\resizebox{.88\linewidth}{!}{%
\begin{tabular}{ccccc}
\hline
\hline
Model                           & Dataset       &Squentropy    & CE  & Square loss             \\ \hline
\multirow{6}{*}{fine-tuned BERT}           &   MRPC          &   \textbf{0.285}   & 0.766              &     0.484           \\
                                &    SST-2 &   \textbf{0.144}           &  0.173               &      0.279          \\
                                &  QNLI    &   \textbf{0.189}          &  0.205
             &      0.241         \\
                                &  QQP     &  0.050          & 0.063               &  \textbf{0.045}              \\
                                &  text5   &    \textbf{0.132}          &   0.167            &   0.147             \\
                                &  text20  &  0.131             &       \textbf{0.08}        & 0.172               \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL\end{tabular}} & text8      &   \textbf{0.149}     & 0.204    &     0.174      \\
                                & enwik8   &    0.156       & \textbf{0.102} &    0.228      \\
                                \hline

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM\\+Attention\end{tabular}} & MRPC        &  \textbf{0.315}    & 0.786 & 0.484          \\
                                & QNLI     &   \textbf{0.198}      & 0.371 & 0.210          \\
                                & QQP      &   0.408      & \textbf{0.352}           & 0.566 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM\\+CNN\end{tabular}}       & MRPC        &   \textbf{0.289}   & 0.383 & 0.322          \\
                                & QNLI     &   \textbf{0.154}     & 0.286  & 0.173         \\
                                & QQP      &    0.279     & \textbf{0.161}           & 0.458 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Attention\\+CTC\end{tabular}}  & TIMIT (PER)   & 0.332   & \textbf{0.249}          & 0.508 \\
                                & TIMIT (CER)  &  \textbf{0.232}   & 0.873  & 0.361          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VGG+\\BLSTMP\end{tabular}}     & WSJ (WER)   &  \textbf{0.147}    & 0.249  & 0.184         \\
                                & WSJ (CER)      &  0.082 & 0.118 & \textbf{0.077}          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VGG+\\BLSTM\end{tabular}}      & Libri (WER)& \textbf{0.117}  & 0.257  & 0.126          \\
                                & Libri (CER) & \textbf{0.125}&0.316  & 0.148           \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Transformer\end{tabular}}      & WSJ (WER) &  \textbf{0.186}    & 0.276    &    0.206   \\
                                & Libri (WER) &  0.168 &  0.232  &   \textbf{0.102}           \\                                
                                \hline
TCNN                            & MNIST          &  \textbf{0.151} & 0.173  & 0.161          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Resnet-18\end{tabular}}     & CIFAR-10     & \textbf{0.147}  &   0.452 &      0.174     \\ 
& STL-10 &   0.413   &   0.376    &  \textbf{0.230} \\ \hline
W-ResNet      & CIFAR-100     &  \textbf{0.164}   &   0.433   &    0.181    \\ \hline
Visual Transformer                     & CIFAR-10    &  0.070    &  0.075     &  \textbf{0.063}         \\ \hline
VGG  & SVHN & 0.283   &   \textbf{0.246}      & 0.307 \\ \hline
\multirow{2}{*}{Resnet-50}      & I-Net (Top-1)  &    \textbf{0.029}    & 0.045 & 0.032          \\
                                & I-Net (Top-5)         & 0.098 &\textbf{0.045}          & 0.126 \\ \hline
\multirow{2}{*}{EfficientNet}   & I-Net (Top-1)  &   \textbf{0.099}     & 0.122          & 0.138 \\
                                & I-Net (Top-5)    & 0.092    &\textbf{0.089}  & \textbf{0.089} \\ \hline
\end{tabular}
}%
\vspace{-4mm}
\end{table}

